NELA-GT-2022: A Large Multi-Labelled News Dataset for The Study of Misinformation in News Articles

In this paper, we present the fifth installment of the NELA-GT datasets, NELA-GT-2022. The dataset contains 1,778,361 articles from 361 outlets between January 1st, 2022 and December 31st, 2022. Just as in past releases of the dataset, NELA-GT-2022 includes outlet-level veracity labels from Media Bias/Fact Check and tweets embedded in collected news articles. The NELA-GT-2022 dataset can be found at: https://doi.org/10.7910/DVN/AMCV2H

==> tex/labels_legend_table.tex <==
\newgeometry{left=2cm, top=1.4cm}

\begin{table*}[!ht]
    \fontsize{9}{9.2}\selectfont  % fontsize, spacing
    \renewcommand{\arraystretch}{1.4}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[t]{L{3.6cm}lL{10.4cm}C{2.5cm}}
        \textbf{Section} & & \textbf{Description} \hfill (NewsGuard points) & \textbf{Coloring} \\ \hline
        %
        NewsGuard 
        & ~~1. & Does not repeatedly publish false content \hfill (22.0)  & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & ~~2. & Gathers and presents information responsibly \hfill (18.0) &  \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & ~~3. & Regularly corrects or clarifies errors \hfill (12.5)  &                                 \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~4. & Handles the difference between news and opinion responsibly \hfill (12.5)  &            \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~5. & Avoids deceptive headlines \hfill (10.0) &                                              \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~6. & Website discloses ownership and financing \hfill (7.5) &                               \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~7. & Clearly labels advertising \hfill (7.5) &                                              \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~8. & Reveals who's in charge, including any possible conflicts of interest \hfill (5.0) &   \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~9. & Provides information about content creators \hfill (5.0) &                             \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& 10. & Aggregated \texttt{score} computed from 1-9 & \includegraphics[width=1.6ex]{fig/colors/green.pdf} - \includegraphics[width=1.6ex]{fig/colors/purple.pdf} ~~ \\
    	& 11. & Column 10 thresholded at 60 points &
    	\includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/purple_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
    	% 
    	Pew Research Center 
    	& 12. & Trust from consistently-liberals & \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 13. & Trust from mostly-liberals & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 14. & Trust from mixed groups & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 15. & Trust from mostly-conservatives & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 16. & Trust from consistently-conservatives & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 17. & Aggregated trust from 12-16 & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
        % 
        Wikipedia 
        & 18. & Existence of source on Wikipedia's list of fake news sources & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
        % 
        Open Sources 
        & 19. & Marked reliable & \includegraphics[width=1.6ex]{fig/colors/green.pdf} \\
        & 20. & Marked blog & \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 21. & Marked clickbait & \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 22. & Marked rumor & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 23. & Marked fake & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 24. & Marked unreliable & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 25. & Marked biased & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 26. & Marked conspiracy & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 27. & Marked hate speech & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 28. & Marked junk science & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 29. & Marked political & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 30. & Marked satire & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 31. & Marked state news & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\ \hline
        %
        Media Bias / Fact Check 
        & 32. & Factual reporting from 5 (good) down to 1 (bad) & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/purple_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 33. & Special label; conspiracy, pseudoscience or questionable source (purple), and satire (orange) &
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 34. & Political leaning / bias from left to right. & 
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/blue_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        Allsides 
        & 35. & Political leaning / bias & 
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/blue_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        BuzzFeed
        & 36. & Political leaning / bias, but only left and right &
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        PolitiFact
        & 37. & Has brought story labelled as "pants on Fire!" &
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 38. & Has brought story labelled as false &
        \includegraphics[width=1.6ex]{fig/colors/purple2_grey.pdf} \\
        & 39. & Has brought story labelled as mostly false &
        \includegraphics[width=1.6ex]{fig/colors/purple_grey2.pdf} \\
        & 40. & Has brought story labelled as half-true &
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 41. & Has brought story labelled as mostly true &
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} \\
        & 42. & Has brought story labelled as true &
        \includegraphics[width=1.6ex]{fig/colors/green.pdf} \\ \hline
        %
        Alexa Ranking & & The Alexa ranking of the source. & Numerical \\ \hline
        %
        \# Articles & & The number of articles collected from the source. & Numerical \\ \hline
        %
        First Observed & & The date of first articles collected from the source. & dd-mm-yyyy \\ \hline
    \end{tabular}
    \caption{Details of the information for sources found in tables \ref{tab:source_labels1}, \ref{tab:source_labels2} and \ref{tab:source_no_labels}. We generally use green-to-purple for good-to-poor reliability/credibility, with grey as inconclusive. For bias we use blue-to-red for left-to-right bias, with grey as unbiased. Orange is used for special cases. In NewsGuard data it represents missing information, in Open Sources it marks auxiliary labels and for Media Bias / Fact Check it marks satire. }
    \label{tab:labelling_explanations}
\end{table*}

\restoregeometry

